Before You Hand Over the Wheel: Evaluating LLMs for Security Incident Analysis

Security incident analysis (SIA) poses a major challenge for security operations centers, which must manage overwhelming alert volumes, large and diverse data sources, complex toolchains, and limited analyst expertise. These difficulties intensify because incidents evolve dynamically and require multi-step, multifaceted reasoning. Although organizations are eager to adopt Large Language Models (LLMs) to support SIA, the absence of rigorous benchmarking creates significant risks for assessing their effectiveness and guiding design decisions. Benchmarking is further complicated by: (i) the lack of an LLM-ready dataset covering a wide spectrum of SIA tasks; (ii) the continual emergence of new tasks reflecting the diversity of analyst responsibilities; and (iii) the rapid release of new LLMs that must be incorporated into evaluations. In this paper, we address these challenges by introducing SIABENCH, an agentic evaluation framework for security incident analysis. First, we construct a first-of-its-kind dataset comprising two major SIA task categories: (i) deep analysis workflows for security incidents (25 scenarios) and (ii) alert-triage tasks (135 scenarios). Second, we implement an agent capable of autonomously performing a broad spectrum of SIA tasks (including network and memory forensics, malware analysis across binary/code/PDF formats, phishing email and kit analysis, log analysis, and false-alert detection). Third, we benchmark 11 major LLMs (spanning both open- and closed-weight models) on these tasks, with extensibility to support emerging models and newly added analysis scenarios.

==> Benign_Sample_Set.tex <==
\subsection{Part II: Alert Triaging Tasks}
% After creating our SIA dataset for evaluating LLMs in investigating malicious activities, we extend our exploration to an equally important challenge: investigating false positive alerts and benign artifacts. 
% As highlighted in \cite{alahmadi202299, yang2024true},
% in real-world environments, security analysts frequently 
% face the burden of detecting a high volume of false alerts 
% generated by various security tools (e.g., Snort \cite{snort}, Suricata \cite{suricata}). 
% % These false positives consume valuable time and resources, as analysts must investigate benign network activity that appears suspicious. 
% To assess how effectively LLMs can assist in this scenario, we evaluate their ability to recognize false positives. 
% and avoid being misled by benign traffic that triggers alerts. 
There is a lack of false alert datasets in a format suitable for LLMs, as well as a lack of benchmarks that directly evaluate their performance in analyzing benign artifacts.
%However, the is a lack of false alert dataset in appropriate form to be fed into LLMs and a lack of existing benchmark directly evaluates LLM performance in analyzing benign artifacts for this purpose.
To address this gap, in our dataset, we  
include benign scenarios (and their corresponding false alerts).
% also to 
% evaluate LLM capabilities in false-positive detection.
Specifically, we focus on network forensics-related tasks using artifacts like network level alerts by IDS (e.g., Snort, \red{Suricata} \cite{snort, suricata}).
% while utilizing the CIC-IDS 2017 Intrusion Detection Evaluation Dataset \cite{cicids2017}. 
% and alert triage and in-depth analysis of benign artifacts. 
We develop the dataset through the following steps 
% as follows.
% : artifact collection, alert generation, and sample set construction 
(as illustrated in Fig. \ref{fig:benign_data_generation}).



\begin{figure}[ht] % Ensures the figure fits within the column
    \centering
    \includegraphics[width=\columnwidth]{images_pdf/Alert_Triage_Dataset_Design.pdf} % Replace with your image file name
    % \vspace{-0.3in}
     \caption{Alert Triage Dataset (Part II) Generation Process.}    
      \vspace{-0.2in}
    \label{fig:benign_data_generation}
\end{figure}

\begin{figure}[ht] % Ensures the figure fits within the column
    \centering
    \includegraphics[width=\columnwidth]{images_pdf/alert.pdf} % Replace with your image file name
    % \vspace{-0.3in}
     \caption{Alert Triage Dataset (Part II) Generation Process.}    
      \vspace{-0.2in}
    \label{fig:benign_data_generation_1}
\end{figure}


\subhead{Artifact Collection} 
% To explore the capabilities of large language models (LLMs) in handling benign artifacts, 
At first,
we utilize the CIC-IDS 2017 Intrusion Detection Evaluation Dataset \cite{cicids2017}, which 
% provides a collection of network traffic data. The dataset 
contains PCAP files spanning five days and including a mix of both benign and malicious traffic. 
The malicious samples cover a range of common attacks, such as web-based attacks, brute force, denial of service (DoS), distributed denial of service (DDoS), infiltration, Heartbleed, botnet activity, and scanning. The traffic from Monday is entirely benign, whereas the remaining days contain a mix of both benign and malicious traffic. To isolate the benign and attack portions from the mixed captures, we use the provided attack timestamps to segment out the mixed traffic.
Unlike previous blue team training platforms \cite{BTLO, CyberDefenders, tryhackme}, the CIC-IDS dataset does not include any natural-language-based predefined scenarios or questions. Therefore, we manually craft scenarios and corresponding questions from the raw PCAPs to evaluate the role of LLMs in the context of investigating normal, non-malicious network traffic, as follows. 
% In the following, we detail our approach for crafting these scenarios and questions.
% based on the CIC-IDS traffic captures. For that, at first we generate alerts from the isolated captures.

\subhead{Alert Sample Generation} Following the above mentioned attack and benign PCAP segmentation, we generate alerts from these PCAP segments for realistic LLM evaluation. For alert generation from segmented PCAPs, we leverage Snort version 3.0 \cite{snort} with default Snort community rules, freely available from the official Snort website. 
% After running Snort alerts, we receive various alerts, including false alerts from benign pcap. 
We use those generated alerts to craft the dataset as follows. 

% We generate a sample set by using two complementary approaches to address different aspects of analyst workflows: \textit{alert triaging} and \textit{deep-dive investigation} (results dicussed in Sec. \ref{sec:benign_result}). Alert triaging evaluates the model's ability to classify alerts as true positives, which is critical for prioritizing analyst workload and reducing time spent on benign activities. Deep-dive investigation assesses whether LLMs can be misled by false positive scenarios when asked to perform detailed analysis of benign artifacts, testing their resilience against confirmation bias and their ability to correctly conclude that suspicious-looking traffic is actually benign.

% Following the attack and benign pcap segmentation, to craft meaningful scenarios and questions, we employ Snort \cite{snort}, one of the most widely used open-source intrusion detection systems (IDS) \cite{murgai2024enhancing}. We utilize Snort version 3.0 along with the default community rules available from the official Snort website. Snort is run on both the benign and attack segments to generate corresponding alerts. 

% \subhead{Sample Generation} To craft the scenarios and questions, we generate a sample set by using two complementary approaches to address different aspects of analyst workflows: \textit{alert triaging} and \textit{deep-dive investigation}. Alert triaging evaluates the model's ability to classify alerts as true positives, which is critical for prioritizing analyst workload and reducing time spent on benign activities. Deep-dive investigation assesses whether LLMs can be misled by false positive scenarios when asked to perform detailed analysis of benign artifacts, testing their resilience against confirmation bias and their ability to correctly conclude that suspicious-looking traffic is actually benign.

% \noindent\emph{\underline{Alert Triaging}}: Alert triaging determines whether generated alerts represent genuine security threats or benign network activity.

\noindent\textit{Scenario Generation}: We incorporate alert descriptions directly into the scenarios,
while maintaining consistency with the Part-I of our dataset. Example: ``The SOC team has received the following alert: \texttt{07/07-08:00:50.818009 [**] [122:1:1] (port\_scan) TCP portscan [**] [Priority: 3] \{TCP\} 192.168.10.3:88 - 192.168.10.5:49175}. A PCAP file has been provided to investigate the alert.''
 % Each scenario follows the format: \textit{``The SOC team has received the following alert: [alert description]. A pcap file has been provided to investigate the alert.
    
\noindent\textit{Question Formulation:} For alert triaging, we formulated a single simple and direct question in a general form: ``Analyze the provided PCAP file and determine if the generated alert is a false positive or true positive.''

\noindent\textit{Ground Truth Labeling:} Using the labeled data from CIC-IDS 2017 dataset, we label alerts for actual attack data as \textit{true positive}, and alerts for benign data as \textit{false positive}. 

% We analyze alert descriptions and corresponding attacker/victim IP addresses to establish truthfulness. True positive samples receive the label \textit{True Positive}, while false positive samples are labeled \textit{False Positive}.

\noindent\textit{Artifact Refinement}: Due to the large size of the PCAP files often containing over 100,000 packets, it is impractical to evaluate LLMs directly on these full captures because of their context limitations \cite{context_limit1, context_limit2}. To address this, we use the alert timestamps to further segment the PCAPs into smaller chunks, each containing approximately 5,000 to 10,000 packets, ensuring that the segments still generate the relevant alerts. Finally, we re-run Snort on these refined segments to verify that the same alerts are still produced, thus confirming the integrity of the segmentation process. The corresponding segmented PCAP files related to each alert are provided to the LLM for analysis.


% commenting out deep-deive for SP submission
% \noindent\emph{\underline{Deep-Dive Investigation}}: Deep-dive investigation mirrors our SIA dataset design approach (discussed in Sec. \ref{sec:dataset}), requiring comprehensive analysis of benign network artifacts.

% \noindent\textbf{Scenario Generation:} To maintain consistency with our SIA dataset design approach, we transform alert descriptions into scenarios with similar tone and abstraction level. Rather than including concrete alert details (e.g., IP addresses, timestamps, port numbers), we extract key behavioral indicators and craft abstract descriptions that mirror our SIA dataset scenarios. We employ Gemini 1.5 Flash \cite{Google_AI} for initial scenario generation using few-shot learning \cite{ma2023fairness} with example scenarios from SIA dataset, the generated alert. Each generated scenario undergoes manual validation and adjustment to ensure alignment with our SIA dataset tone. Example: The alert \textit{``07/07-08:00:50.818009 [**] [122:1:1] (port\_scan) TCP portscan [**] [Priority: 3] \{TCP\} 192.168.10.3:88 -> 192.168.10.5:49175''} becomes: \textit{An analyst detects unusual network activity suggesting that an internal host is scanning another internal system, raising concerns of potential port scanning activity. A pcap file, capture.pcap, has been provided to determine if this is benign network behavior or an indicator of compromise.}

% \noindent\textbf{Question Format:} We design three distinct questioning approaches for deep-dive investigation, each targeting different aspects of LLM reasoning and bias detection:

% \begin{itemize}[leftmargin=*, itemsep=0pt, topsep=0pt]
%     \item \textbf{Assumption-Based Questions}: Inspired and aligned with blue team training platforms, these questions assume the incident's validity and seek direct investigative details. They presuppose malicious activity and request specific evidence (IPs, files, etc.). Example: \textit{What is the IP address responsible for conducting the port scan activity?}
    
%     \item \textbf{Reasoning-First Questions}: Aligned with our debiasing approach taken in developing SIA dataset, these questions prompt LLMs to assess incident validity before providing details. They encourage critical analysis rather than assumption. Example: \textit{Is there any indication of port scanning activity in the network traffic? If so, what is the IP address?}
    
%     \item \textbf{Validation-Only Questions}: These questions test whether LLMs are influenced by evidence-seeking prompts by focusing solely on incident truthfulness without requesting specific indicators. Example: \textit{Is there any indication of port scanning activity in the network? Answer with yes/no.}
% \end{itemize}

% \noindent\textbf{Ground Truth Labeling:} As for deep-dive investigation, the alerts are generated from benign samples, so by definition, the ground truth answer for every question (finding malicious IPs, attack scans, or harmful downloads) becomes \textit{no such entity}.

% % As for deep-dive investigation, the alerts are generated from benign samples, The ground truth for each query is set to \textit{no such entity.}

% \noindent\textbf{Artifact}: Corresponding segmented pcap files related to each alert are provided to the LLM for analysis in the same way, we perform for the alert-triaging. 


This part of the dataset has 30 false positive 
and five true positive alert scenarios in network forensics context
with more scenarios
and contexts to be added in the future. \red{Overall, our alert triage dataset includes both TP and FP from network level analysis (IDS alerts verification) to mirror SOC workflow and SIA dataset includes TPs using richer artifacts for in-depth analysis\cite{mitre_11, alahmadi202299}.}
The ethical considerations for our dataset are in Appendix~\ref{appendix:ethics}.
% five true positive alerts and 30 false positive alert scenarios. 

% For deep-dive investigation, we have crafted ten scenarios, generating 39 questions focused on investigative questions such as, attacker and victim IP identification, scan classification, file extraction, leaked data information, command execution analysis.

==> Discussion.tex <==
\section{Discussion} \label{sec:discussion}

\subhead{Model Adaptability and Integration Challenges} \label{sec:newmodel_adaption}Our evaluation framework is designed to be adaptable, supporting various LLMs compatible with LangChain/LangGraph frameworks to enable seamless integration and testing. After developing our SIA agent, we integrate models such as Llama-3.1-8B, Llama-3.1-70B, Llama-3.1-405B, Claude-4.5-Sonnet, Claude-3.5-Sonnet, Gemini-1.5-pro, GPT-4o-mini, GPT-4o, o3-mini, GPT-5.
Although most models are instruction-tuned \cite{shi2024instruction} and generally adhere to prompts, LLM agents occasionally fail to follow instructions, especially the smaller models like Llama 8B variants, leading to errors or incomplete task execution \cite{follow_instructions}. 
%Although most models are instruction-tuned \cite{shi2024instruction} and generally follow prompts, LLM agents occasionally fail to follow instructions, resulting in errors or incomplete tasks \cite{follow_instructions}. Specifically, Llama models, especially variant 8B, are less capable for agentic-based frameworks \cite{llama-8b-issue}, as they do not use functions and tools properly and have less precision in multi-turn problem-solving tasks \cite{berkley}, as is also evident from our evaluation result in Sec. \ref{sec:RQ1-4}. 
However, to maintain consistency, in this research, all models are evaluated using the same prompts and agent structure (zero-shot ReAct prompting with tool usage instructions and consistent prompt formatting) and we rerun any incomplete runs if any. Differences in model behavior reveals several integration challenges. First, \textit{prompt updates: } We notice that o3-mini struggle with function calling. Based on community discussions \cite{o3_mini_forum_post}, we adjust our prompts to improve the consistency of o3-mini. Second, \textit{jail breaking: } GPT-5 flagged outputs as policy violations. Following previous work \cite{deng2024pentestgpt}, we apply jail breaking technique to bypass these restrictions for the benchmarking.  


% Differences in model behavior revealed several integration challenges: First, \textit{prompt formatting issues: } some models failed to interpret standard prompt structures and required prompt modifications to function correctly. Second, \textit{functionality limitations: } certain models could not handle the provided functions as expected and need architectural simplifications.

\subhead{Mitigating LLM Data Contamination Risk} 
\red{There is a possibility that the evaluated LLMs have seen the write-ups of the SIABench scenarios in their training data. 
%\red{%It is possible that LLMs used by \oursolution were trained on walkthroughs of the benchmark machines, which could invalidate evaluation results.
To mitigate such data contamination risk, we adopt three strategies. First, we pre-process the data to minimize triggers that might cause the LLM to retrieve memorized content \cite{kerr2025icarus}, as discussed in section \ref{sec:dataset}. Second, we follow vendor guidance (OpenAI, Microsoft, Anthropic \cite{anthropic, OpenAI} indicating that model knowledge is limited to its training cutoff unless augmented through tools (e.g., RAG, web access) or explicit fine-tuning. Accordingly, we evaluate models using tasks released after their respective training cutoff dates, as discussed in Section \ref{sec: evaluation_nn}.
%To address this, we apply three methods. First, we preprocess our data that can trigger the LLM to fetch answers from its memorized data \cite{kerr2025icarus} as discussed in Sec. \ref{sec:dataset}. Second, we follow vendor guidance (OpenAI, Microsoft, Anthropic \cite{anthropic, OpenAI}) that model knowledge ends at its training cutoff unless augmented via tools (e.g., RAG and web access) or explicit fine-tuning and evaluate the models with tasks that are released after their training cut-off data as discussed in Section \ref{sec: evaluation_nn}. 
Third, we assess whether the LLMs underwent targeted training by querying them by providing scenario name, platform name and raw questions (without the answers) for detailed information about specific scenarios. These conventions have been used in previous works such as PentestGPT, Cybench and IRCopilot \cite{deng2024pentestgpt, zhang2024cybench, lin2025ircopilot}.} 

\subhead{Guided nature of Investigative Question} \red{As we discussed before, our dataset  structure may not fully capture the unguided, exploratory nature of full-scale expert-level SIA
tasks, but we selected a diverse SIA suite (Network/Memory Forensics, Malware, Phishing, and Log Analysis) grounded in training materials used to prepare junior analysts for 5-30 years, ensuring real-world relevance. Therefore, we use guided questions like those given to junior analysts to focus the model’s responses and enable partial evaluation of task-solving capabilities. Moreover, we also explored fully open-ended prompts, LLMs often produced unfocused or irrelevant outputs, not having specific ground truths, making accurate benchmarking difficult.}

\subhead{Security Tool Selection} \red{As discussed in Section \ref{sec:dataset}, we recommend some of the security tools to the LLM to analyze following blue team training platform standards \cite{CyberDefenders, BTLO, tryhackme}. We acknowledge that tool selection depends on context and rarely has a single “right” choice. We do not bind the LLMs to use only the mentioned tools. The LLMs were instructed to install additional tools by adding \texttt{sudo} in the beginning.}

\red{All security tools run inside a controlled Kali Linux VM. The preinstalled packages cover common utilities. For most cases the latest version of the recommended tools is installed, as we do not mention any specific version numbers. LLMs also install the latest version by using default installation commands (which install latest version of the tools). And the raw CLI outputs are preserved and cleaned (removal of non-printable ASCII characters) to provide the tool output as a human-readable format.}


\subhead{Summarizer Module} 
% To address context limitations and better planning of agent, a summarizer module is implemented, extending outputs up to a 640k context limit for tasks exceeding the 128k limit, such as memory forensics and PCAP log analysis. For cases beyond this, the module suggests iterative attempts with the message, ``Find a way to solve the problem more efficiently''.
To address context limitations and improve the agent’s planning capabilities, we implemented a summarizer module that allows the system to handle tasks whose input size exceeds the base context limit (e.g., 128k for \textit{GPT-4o}), such as memory forensics or PCAP log analysis. In our implementation, the summarizer is configured to extend the usable context up to approximately 640k tokens. This value reflects a design choice of our summarizer module, which can operate beyond this threshold depending on how it is configured. For inputs that still exceed the configured limit, the module instructs the agent to attempt a more efficient approach through an iterative message such as “Find a way to solve the problem more efficiently.”

==> Old_Methodology_Dataset.tex <==
%\section{Methodology}
\section{Security Incident Analysis (SIA) Dataset}
\label{sec:dataset}

This section presents our security incident analysis dataset.

\red{\subsection{Dataset Design} (Not sure where to put and how to put about the dataset design justification)} Our dataset is designed from the perspective of a blue team trainee analyst in a controlled training environment, where tasks are based on real-world incident scenarios. In actual analyst training environments—such as SANS courses (e.g., FOR572) \cite{sans_course}, different certification exams (e.g. PSAA) \cite{psaa, blue_certification}, training platforms like LetsDefend, CyberDefenders \cite{Blue}, CTF like exercises \cite{ctf_1, ctf_2}—analysts are not operating blindly. They are guided by structured, goal-driven objectives that reflect operational threat hunting and incident response processes.

Related literature also supports domain-specific evaluations of LLMs using standardized, goal-driven question formats. For instance, in the medical domain, LLMs have been evaluated using USMLE exam questions \cite{usmle}, while in cybersecurity, models have been assessed against Cisco certification exams \cite{tann2023using}. Offensive security datasets and benchmarks such as PentestGPT, CyBench, and Intercode \cite{deng2024pentestgpt, zhang2024cybench, yang2023language} leverage gamified CTF-style tasks to evaluate LLM capabilities. In contrast, our benchmark focuses on evaluating LLMs as junior blue team analysts, with each scenario framed through investigative, guided questions that reflect the analytical reasoning processes used by practitioners.


\subhead{Dataset Selection}


\red{\subsection{Dataset Design} (Not sure where to put and how to put about the dataset design justification)} Our dataset is designed from the perspective of a blue team trainee analyst in a controlled training environment, where tasks are based on real-world incident scenarios. In actual analyst training environments—such as SANS courses (e.g., FOR572) \cite{sans_course}, different certification exams (e.g. PSAA) \cite{psaa, blue_certification}, training platforms like LetsDefend, CyberDefenders \cite{Blue}, CTF like exercises \cite{ctf_1, ctf_2}—analysts are not operating blindly. They are guided by structured, goal-driven objectives that reflect operational threat hunting and incident response processes.

Related literature also supports domain-specific evaluations of LLMs using standardized, goal-driven question formats. For instance, in the medical domain, LLMs have been evaluated using USMLE exam questions \cite{usmle}, while in cybersecurity, models have been assessed against Cisco certification exams \cite{tann2023using}. Offensive security datasets and benchmarks such as PentestGPT, CyBench, and Intercode \cite{deng2024pentestgpt, zhang2024cybench, yang2023language} leverage gamified CTF-style tasks to evaluate LLM capabilities. In contrast, our benchmark focuses on evaluating LLMs as junior blue team analysts, with each scenario framed through investigative, guided questions that reflect the analytical reasoning processes used by practitioners.
% the key features of our Security Incident Analysis (SIA) dataset
% for LLM evaluation
% and how it is built.

% We created the SIA benchmark dataset by carefully curating diverse SIA tasks from from real-world scenarios. We also conducted a validation procedure of the dataset involving security experts. The following subsections present the key features of the dataset and it's development procedure.

\subsection{Dataset Features}

Our dataset incorporates several key features designed to evaluate the capabilities of LLMs for real-world SIA tasks:

\begin{itemize}[leftmargin=*, itemsep=0pt, topsep=0pt]
    \item \textbf{Diverse SIA Tasks:} 
    To capture the diverse nature of the SIA tasks,
    we include four major categories of security incident scenarios:
    \emph{network forensics} (covering malicious traffic analysis),  \emph{memory Forensics} (covering memory dump and disk analysis),\emph{malware analysis} (covering file dissection, code review, and script analysis), and \emph{miscellaneous} (covering other tasks, including phishing email/kit analysis, and log analysis).
    % The dataset includes a diverse set of security incident scenarios covering key SIA tasks such as network and memory forensics, malware analysis, phishing kit, and log analysis.
    The tasks also involve 15 security tools reflecting real-world scenarios.
    This is further detailed in Section~\ref{sec:labeling}.
    % (as detailed in Section \ref{sec:taskdesign}).
    
    \item \textbf{Task Difficulty Level:} 
    Security incident analysis tasks often vary in their 
    difficulty level \cite{karie2015taxonomy}. To include this factor in testing basic-to-advanced capabilities of LLMs while varying task complexity,
    we consider SIA tasks covering three different difficulty levels:
    easy, medium, and hard; as detailed in Section~\ref{sec:labeling}.
    % To build a realistic dataset for evaluating 
    % The benchmark is designed to test basic and advanced capabilities of LLMs on tasks of varying complexity so as to ensure a wide applicability. 
    
    \item \textbf{Work-flow Alignment with Real-world:} The SIA tasks of our  dataset are designed to reflect the workflow of real-world security analysts by following the adversarial tactic alignment (e.g., reconnaissance, initial access) outlined by CISA \cite{cisa}, and foundational investigative questions (e.g., \emph{who}, \emph{what}, \emph{how}) of SANS guidelines  \cite{dfir}. For example, the question, \emph{which IP is responsible for port scanning activity?}, facilitates the identification of the \emph{who} behind the attack while also allowing an investigation into the reconnaissance phase of the adversary's attack tactics, thus aligning with both investigative frameworks.
    
    \item \textbf{Validation by Security Professional and Researchers:} A rigorous multi-step validation process was carried out on the dataset, involving three groups of security experts: academic researchers, federal government researchers, and federal government security professionals. In the first phase, each task is evaluated by human experts to ensure that it could be realistically solved using command-line tools. In the second phase, an in-depth validation process is undertaken to minimize bias and enhance the dataset's alignment with real-world analyst workflows. This involved paraphrasing questions to remove assumptions and specific numerical values, making them more open-ended, and ensuring clarity and structure. Additionally, the dataset's labels and ground-truth answers are carefully reviewed for accuracy and consistency.
%We do a multi-step validation process to ensure the quality of our dataset, such as ensuring each of the scenario can be solved with command-line-based tools, removing bias from the questions (e.g., presumptions), ensuring the answers are correct, structuring the dataset format, etc., covering multiple domains of SIA tasks.
     % \item \textbf{Adversarial Tactic Alignment}: Tasks are mapped to adversarial tactics (e.g., reconnaissance, initial access) in line with CISA guidelines \cite{cisa}, mapping to critical questions like \textit{“What method is used for reconnaissance?”}
    % \item \textbf{Foundational Investigative Questions}: Our benchmark dataset reflects investigative questions (e.g., “who, what, how”) essential to security-incident analysis, following SANS guidelines. For example, "who is the attacker?" or "what file was executed or delivered?"
    % \item \textbf{Balanced Questioning Approach}: In our dataset, we provide questions with clear ground truth without being overly generic or overly specific. For instance, a question like, “Is there any abnormal activity happening here?” is overly generic and lacks a specific ground truth for assessment. Conversely, a question such as, “What are the two attackers’ IP addresses?” is overly specific and may limit the scope of analysis. Instead, we aim for a balanced questioning approach. For example, a question like, “Are there any IP addresses that have been interacting with the server recently and that seem suspicious? If so, what are they?” provides a clear ground truth for evaluation while allowing the model to analyze patterns and identify suspicious activity without being very specific.
\end{itemize}


\subsection{Dataset Development} \label{sec:dataset_design}
We develop this dataset in three phases: data collection, data refinement, and data labeling
% The development process of our benchmark is 
(as shown in Figure \ref{fig:Question_Formation}).

\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{images_pdf/dataset_design.pdf}
    \vspace{-0.3in}
    \caption{SIA Dataset Design and Development Process.}
    \vspace{-0.2in}
    \label{fig:Question_Formation}
\end{figure*}
\subhead{Data Collection}
%\subhead{Data Collection}
%\subhead{Data Collection} 
We collect publicly available SIA scenarios from well-known cyber defense and blue team training platforms \cite{Blue}, such as CyberDefenders \cite{CyberDefenders}, Blue Team Labs Online \cite{BTLO}, and TryHackMe \cite{tryhackme}. The selected scenarios cover a wide range of SIA tasks, including the tasks related to forensics, malware analysis, phishing analysis, log analysis, etc., with a variety of security incidents, including ransomware attacks, web server compromises, phishing-driven malware infections, drive-by download attacks, Linux server compromises, port scanning attack. The selected scenarios span multiple infrastructure levels, e.g., network, operating system, memory, file system, and application-level files \textit{(.pdf, .xml, .eml)}, to comprehensively address various sources of evidence \cite{dfir} related to security incident analysis tasks. 
% The selected scenarios also span multiple infrastructure levels, including network, operating system, memory, file system and application-level files (.pdf, .xml, .eml), to comprehensively address different aspects of security incident analysis. 
% Each scenario includes a description, artifacts such as .pcap, .mem, .eml files, usable security tools, and key investigation questions for conducting the analysis. 
Each scenario includes a description, artifacts, such as \textit{.pcap, .mem, .eml} files, a set of example security analysis tools to analyze with, and key investigation questions for conducting the analysis. 

{\subhead{Data Refinement and Task Design}}
%\subhead{Data Refinement and Task Design}
\label{sec:taskdesign}
%\subhead{Data Refinement and Task Design} 
% After collecting the scenarios, we refine and enhance data to ensure its quality and relevance following the recommendation of a security professional in our team. We design the SIA tasks containing the following components:
After collecting the scenarios, we refine and enhance data to ensure its quality and relevance by adhering to standard recommendations \cite{prompt_bias, potential_bias, satvaty2024undesirable}, alongside input from a security professional in our team. This process, along with the design of the SIA tasks, is further detailed within the following components of the SIA tasks:

\red{\noindent\emph{\underline{Scenario Description.}} }
We extract the description of each scenario 
from their original sources (e.g., cyber defense and blue team training platforms)
to 
provide a very brief overview of the incident, such as what happened, the behavior being observed, or the type of analysis involved. For example:
\textit{"An analyst detects unusual network activity suggesting that an internal host is scanning another internal system, raising concerns of potential port scanning activity. A PCAP file, capture.pcap, has been provided to determine if this is a benign network scan or an indicator of compromise."}

However, we pre-process the scenario descriptions collected from various data sources to ensure consistency and reduce the likelihood of memorized responses. Each scenario is rephrased in two main ways. First, we paraphrase the entire scenario using the Gemini 1.5 Flash API \cite{Google_AI}. We use the following prompt: \textit{Paraphrase the following paragraph, keeping the original meaning intact and maintaining approximately the same length. Do not add or remove any key ideas. Use natural, clear language: "[Insert the scenario description here]"}. In addition, we remove specific identifiers from the scenarios, such as company names and user names, and replace them with generalized terms like \textit{a company} or \textit{an employee}. All these efforts are made to avoid direct matches with training data, reducing the chance of memorized responses \cite{code_analysis}. Second, we reduce unnecessary context by removing lengthy background descriptions, such as detailed attack vector explanations, which are not essential to the core investigative content. This ensures the model remains focused on relevant analytical information.

% However, sometimes the original description of the scenario
% does not explain it properly. For instance: the description, \textit{"Put your phishing analysis skills to the test by triaging and collecting information about a recent phishing campaign,"} misses the specific details of a scenario. 
% To overcome this issue, we leverage GPT-4o \cite{ChatGPT} for its advanced natural language processing capability to paraphrase it by providing contextual and scenario-specific inputs to enrich the description. For instance, the previous description is paraphrased to, \textit{"A user working at an organization has reported a suspicious email that he believes might be a phishing attempt. Following the company protocol, the user forwarded the email to the Security Operations Center for further investigation."} This ensures more detailed, clear, and actionable descriptions of scenarios.

% of those scenarios are paraphrased wherever necessary to improve the clarity.

\noindent\emph{\underline{Artifacts and Files.}} 
% The artifacts and necessary files for each scenario are extracted from their original sources to facilitate the analysis process. The original filenames and artifacts are renamed following the recommendation of our security professional team member to remove potential bias of triggering LLMs to retrieve memorized answers without conducting actual investigations. 
The original filenames and artifacts for each scenario are renamed using a generalized pattern, such as changing \texttt{lala.pcap} or \texttt{steal.pcap} to neutral names like \texttt{capture.pcap}, based on the findings from a prior work \cite{code_analysis} and recommendations from our security professional team, preventing LLMs from relying on pre-trained knowledge to retrieve memorized answers \cite{daghmehchi2022memory}, thereby conducting actual investigations on the artifacts.

\noindent\emph{\underline{Tools.}} 
% The security tools that can be used to analyze the files and artifacts to find answers are listed to the investigative questions (that are explained later). We ensure that the tasks can be completed with the command line tools since LLMs are not yet capable of using the Graphical User Interface (GUI) of tools.  However, our autonomous agent (described in Section~\ref{sec:agent}) is not restricted to the tools provided here and is equipped with the ability to install and utilize other tools as needed.
The security tools are given as suggestions for analyzing files and artifacts to find out the answer for investigative questions (discussed later), selected through a review of forensic guides \cite{dfir}, writeups \cite{caruso2024cyberchallenge}, and manual workflows. We ensure that the tasks can be completed with the command line tools since LLMs are not yet capable of using the graphical user interface (GUI) of tools like humans do. However, our autonomous agent (described in Section~\ref{sec:agent}) is not restricted to these suggested tools and is equipped with the ability to install and utilize other tools as needed.

\red{\noindent\emph{\underline{Questions.}} }For each scenario, several investigative questions are provided to understand the scope of the incident and guide the analysis. An important limitation with the original questions is that they contain biases that might nudge the LLM toward a predefined conclusion \cite{prompt_bias, potential_bias}. To address this limitation and create more realistic evaluation conditions, we systematically reformed the original questions using four key strategies:

\noindent\textbf{Open-ended Reformulation:} To encourage evidence-based reasoning and avoid assumptions, we rephrase fact-based questions as analytical prompts. For instance, the raw question \textit{"What is the IP responsible for conducting the port scan activity?"} presumes the existence of port scanning. Instead, we ask \textit{"Is there any evidence of port scanning in the network traffic? If so, what is the IP address responsible for the scanning activity?"} This encourages the model to verify suspicious activity before identifying the IP.


% \textbf{Open-ended Reformulation:} To encourage evidence-based reasoning and avoid assumptions in analysis, we reformulated direct fact-retrieval questions into open-ended analytical queries. For instance, the raw question \textit{"What is the IP responsible for conducting the port scan activity?"} presumes the existence of port scanning. Instead, we ask \textit{"Is there any evidence of port scanning in the network traffic? If so, what is the IP address responsible for the scanning activity?"} This reframing prompts the model to first assess the presence of suspicious activity before identifying specific entities, fostering a more robust and investigative approach.

\noindent\textbf{Assumption removal:} We eliminate specific keyword assumptions that could bias model responses. Questions like \textit{"What's the invoked PowerShell script used by the attacker for dumping credentials?"} are paraphrased to \textit{"Is there any evidence of credential dumping by the attacker? If so, is there any invoked script used by the attacker for dumping credentials?"} This prevents the model from being biased with technology-specific terms (e.g. limiting to PowerShell).

\noindent\textbf{Numeric neutrality:} We remove predetermined quantities to allow models to determine numbers based on evidence. Rather than asking \textit{"What are the attacker's two IP addresses?"}, we ask \textit{"Can you identify if there are any IP addresses that have been interacting with the server recently and that seem to be suspicious?"} This prevents leading the model with fixed expectations.

\noindent\textbf{Analysis-focused filtering:} We exclude questions requiring external knowledge or memorized facts, such as CVE numbers or ransomware family names. This ensures evaluation focuses on the model's analytical capabilities with available evidence rather than recall of external databases.

\red{(Need to address the limitation in another way)} These paraphrasing strategies yield questions that more closely mirror real-world analysis, where investigators must collect evidence without assuming specific facts. Despite our efforts to reduce bias, some inherent bias remains in the question design. Real cybersecurity investigations typically follow a tree-like exploration pattern with frequent dead ends and backtracking, whereas our sequential evaluation enforces a more linear structure. While the paraphrased questions are more open-ended, they still guide analysis in specific directions rather than allowing entirely free exploration. This structured approach is necessary to create a standardized benchmark that enables systematic comparison of model capabilities. Although this design may not fully capture the non-linear, exploratory nature of actual incident response workflows, it reflects how analysts are trained and assessed in practical settings. It keeps a balance between open-ended reasoning and consistent evaluation, preserving the core analytical challenges of real-world security investigations.




% These paraphrasing strategies result in questions that better reflect real-world digital forensics scenarios, where investigators must identify suspicious activities without predetermined assumptions about attack vectors, tools, or quantities involved. Despite our efforts to reduce bias through systematic approach, our question design retains inherent limitations. The sequential nature of our evaluation creates a chain-like structure that does not fully capture the tree-like, exploratory nature of real cybersecurity investigations, where analysts frequently encounter dead ends and must backtrack or explore alternative paths. Additionally, our paraphrased questions, while more open-ended, still guide the analysis toward specific investigative directions rather than allowing completely unconstrained exploration. This structured approach is necessary for creating a standardized, reproducible benchmark that enables systematic comparison of model capabilities, but it necessarily constrains the evaluation to predetermined analytical pathways that may not reflect the full complexity and flexibility required in real-world incident response.

% For each scenario, several investigative questions are provided to understand the scope of the incident and guide the analysis. An important limitation with the original questions is that they contain biases that might nudge the LLM toward a predefined conclusion \cite{prompt_bias, potential_bias}. For instance, investigative questions, such as, \emph{"what are the attacker's two IP addresses?"} or \emph{"provide the name of the compressed file downloaded by the attacker,"} are problematic. They presume certain information, such as the specific number of IP addresses or the existence of a download of a compressed file. As a result, even if there are more or fewer than two IP addresses, the LLM would attempt to find exactly two, limiting the analysis scope by embedding conclusions within the questions, which is not reflective of real-world investigative scenarios. To overcome this limitation, guided by the insights from security professionals, we systematically review and update the questions to remove implicit bias while maintaining clarity. For instance, the first question is revised to \emph{"are there any IP addresses that have been interacting with the server recently and that seem suspicious?} If so, what are they?" This approach of forming questions avoids making assumptions and allows for a more open-ended investigation while still being specific enough to find a ground truth for the questions. 



\noindent\emph{\underline{Ground-truths.}} Finally, ground truths are needed for the evaluation process. We derive the answers (a.k.a. ground-truths) to the questions associated with the scenarios from publicly available write-ups \cite{caruso2024cyberchallenge} and also manually analyze the artifacts using different tools to find and verify the ground truth for each scenario for paraphrased questions. 

% \textit{Note: We observed that when specific questions like “What are the attacker's two IP addresses?” are asked, LLMs can identify two IP addresses. However, when these biases are removed, and more open-ended questions are used, LLMs often identify only one IP address.}

\subhead{Data Labeling}
%\subhead{Data Labeling}
\label{sec:labeling}
%\subhead{Data Labeling} 
After creating the tasks in the aforementioned design, we assign category and difficulty levels to each scenario. The questions of each scenario are also labeled with an \emph{adversarial tactic} \cite{mitre} following CISA's outline \cite{cisa, cisa_tactic}. By using these labels, the dataset facilitates more precise evaluation of how well LLMs can handle tasks from different categories with different difficulty levels.

\noindent\emph{\underline{Difficulty Level.}}
%\textit{\textbf{Difficulty Level:}} 
% We select tasks and scenarios with varying complexity levels to reflect the challenges faced by analysts, ensuring a comprehensive dataset. The scenarios are categorized into easy, medium, and hard categories, covering a range of difficulties that are usually encountered in incident analysis.
We consider the difficulty level of each scenario based on the original sources, which is categorized into easy, medium, and hard levels aligning with other work \cite{deng2024pentestgpt}. This range of difficulty reflects the challenges typically encountered in SIA tasks, ensuring a comprehensive dataset.

\noindent\emph{\underline{Task Category.}}
%\textit{\textbf{Task Category:}} 
We categorize each scenario based on the type of task it performs, specifically based on the type of artifact being analyzed. For instance, scenarios involving PCAP files fall under network forensics, while those analyzing memory dumps or image files are categorized under memory forensics. The categorization is intended for grouping  together relevant tasks and to show that different areas of expertise required to solve different category of tasks \cite{dfir}. The types of tasks included in each category are described below:


\begin{table}[htp]
\vspace{-0.1in}
\scriptsize
\centering
\renewcommand{\arraystretch}{1} % Standard row height
\setlength{\tabcolsep}{1pt} % Reduce column padding
\begin{tabular}{|p{2cm}|p{1.2cm}|p{4.8cm}|}
\hline
\textbf{Category} & \textbf{Scenarios (Questions)} & \textbf{Different SIA tasks} \\ \hline

\textbf{Network Forensics} 
    & \multirow{6}{*}{7 (73)} 
    & Analysis of Phishing-Driven Malware Infection \\  
    & & Analysis of Internal Port Scanning Attack \\  
    & & Analysis of Drive-By Download Attack \\  
    & & Analysis of Ransomware Attack \\  
    & & Analysis of Lateral Movement Activity \\  
    & & Analysis of Unknown Malicious Activity \\
\hline

\textbf{Memory Forensics} 
    & \multirow{3}{*}{6 (49)} 
    & Analysis of Linux Server Compromise \\
    & & Analysis of Phishing-Driven Malware Infection \\
    & & Analysis of Malware Intrusion \\  
\hline

\textbf{Malware Analysis} 
    & \multirow{5}{*}{5 (46)} 
    & Analysis of Binary File \\  
    & & Analysis of Malicious Static Code \\  
    & & Analysis of XML Doc File \\  
    & & Analysis of Ransomware Attack-Related Script \\  
    & & Analysis of Malicious EXE file \\  
\hline

\textbf{Miscellaneous} 
    & \multirow{3}{*}{3 (25)} 
    & Analysis of Phishing Email \\  
    & & Analysis of Typosquatting-Related Phishing Kit \\  
    & & Analysis of Server Compromise (via RCE) Logs \\  
\hline

\end{tabular}
\vspace{0.1in}
\caption{Summary of Different Scenario Categories and SIA Tasks.}
\vspace{-0.1in}
\label{tab:scenario_summary}
\end{table}


\begin{itemize}[leftmargin=*, itemsep=0pt, topsep=0pt]
    \item \textbf{Network Forensics}: includes tasks requiring the LLMs to analyze network traffic, such as, PCAP files.
    \item \textbf{Memory Forensics}: includes tasks requiring the LLMs to inspect disk images or examine memory dumps.
    \item \textbf{Malware Analysis}: includes tasks, such as, malicious file analysis (PDF, XML, binary, etc.), static code review, or inspecting ransomware scripts, etc. 
    \item \textbf{Miscellaneous}: includes tasks such as the analysis of phishing e-mails, log files, and phishing kits.
\end{itemize}

\noindent\emph{\underline{Adversarial Tactic Category.}}
To reflect the investigative intent behind each question, we categorize them according to the adversarial tactics defined in the MITRE ATT\&CK Framework \cite{mitre}. Leveraging data sources, the MITRE ATT\&CK Framework, and CISA guidelines \cite{cisa_tactic}, we manually annotate each question with the corresponding tactic it seeks to uncover. These annotations are designed to align with real-world cybersecurity investigations and follow the investigative workflows outlined in widely adopted frameworks, such as those provided by NIST \cite{nist} and CISA playbooks \cite{cisa}.

The labeling process involves uncovering the adversary’s behavior and reasoning about their likely goals \cite{cisa_tactic} through the investigative question. For instance, the question, \emph{"Is there any evidence of port scanning in the network traffic? If so, what is the IP address responsible for the scanning activity?"}, is focused on detecting \emph{port scanning activity}, which is a technique used by adversaries to gather information about open ports and services on a target network. According to the MITRE ATT\&CK \cite{mitre} framework, this behavior maps to the Reconnaissance tactic (TA0043) and thus labeled with the Reconnaissance tactic because the adversary's goal is to collect critical information to facilitate further exploitation. This aligns with the MITRE ATT\&CK framework's classification and the purpose of the observed behavior.
Some questions do not fall into any distinct tactic, for example, investigative questions like identifying the timestamp of a capture or determining the operating system used by the victim. Therefore, for such questions, the tactic fields are left empty. The list of labeled adversarial tactics along with their corresponding sub-tasks is presented in Appendix Table \ref{tab:tactictasks}.


% Table~\ref{tab:scenario_summary} summarizes the dataset.
% The resulting dataset contains 21 cyber incident scenarios that, in total, contain 193 questions. These scenarios are meant to address core security incident analysis tasks, including different categories and different difficulty levels of questions to evaluate the LLMs. While there are other benchmarks such as  \cite{deng2024pentestgpt, zhang2024cybench, gioacchini2024autopenbench} to evaluate the LLMs in offensive tasks, \cite{code_analysis} for analyzing obfuscated code, \cite{alam2024ctibench} for evaluating cyber threat intelligence-related tasks, our dataset is focused on exploring the capabilities of LLMs in SIA tasks. Our dataset is available at the following link: \url{https://github.com/llmslayer/SIA\_Dataset}.


\red{\subsection{False Positive Sample Set (need to change the title)}}

After creating our SIA dataset for evaluating LLMs on investigating malicious activities, we explore their performance on a different but equally important challenge: investigating false positive alerts and artifacts. Security analysts in real-world environments face a major challenge: they receive numerous false alerts from security tools, such as, Snort \cite{snort} and Suricata \cite{suricata} daily \cite{alahmadi202299, yang2024true}. These false alerts waste time and resources as analysts must investigate benign network activities that appear suspicious. To understand how well LLMs can help with this problem, we evaluate their ability to correctly identify false positives and avoid being misled by benign network traffic that triggers security alerts. We develop a small set of data in three phases: artifact collection,
alert generation, and sample set generation (as shown in Figure \ref{fig:benign_data_generation}).

\begin{figure}[ht] % Ensures the figure fits within the column
    \centering
    \includegraphics[width=\columnwidth]{images_pdf/benign.pdf} % Replace with your image file name
    % \vspace{-0.3in}
     \caption{Benign Sample Set Generation Process}    
     % \vspace{-0.2in}
    \label{fig:benign_data_generation}
\end{figure}

\subhead{Artifact Collection} To explore the capabilities of large language models (LLMs) in handling benign artifacts, we focus on network forensics-related tasks having artifacts like PCAP files. Specifically, we utilize the CIC-IDS 2017 Intrusion Detection Evaluation Dataset \cite{cicids2017}, which provides a comprehensive collection of network traffic data. The dataset contains PCAP files spanning five days and includes a mix of both benign and malicious traffic. The attack samples cover a range of common attacks, such as web-based attacks, brute force, denial of service (DoS), distributed denial of service (DDoS), infiltration, Heartbleed, botnet activity, and scanning. The traffic from Monday is entirely benign, whereas the remaining days contain a mix of both benign and malicious traffic. To isolate the benign and attack portions from the mixed captures, we use the provided attack timestamps to segment out the mixed traffic.

Unlike our attack-oriented dataset, the CIC-IDS dataset does not include predefined scenarios or questions. Therefore, we manually craft scenarios and corresponding questions from the benign portions of the dataset to evaluate the role of LLMs in the context of investigating normal, non-malicious network traffic. In the following sections, we detail our approach for constructing these scenarios and questions based on the CIC-IDS traffic captures. For that, at first we generate alerts from the isolated captures.

\subhead{Alert Generation} Following the segmentation, to craft meaningful scenarios and questions, we employ Snort \cite{snort}, one of the most widely used open-source Intrusion Detection Systems (IDS) \cite{murgai2024enhancing}. We utilize Snort version 3.0 along with the default community rules available from the official Snort website. Snort is run on both the benign and attack segments to generate corresponding alerts. 

\subhead{Sample Generation} Due to the large size of the PCAP files—often containing over 100,000 packets—it is impractical to evaluate LLMs directly on these full captures because of their context limitations. To address this, we use the alert timestamps to further segment the PCAPs into smaller chunks, each containing approximately 5,000 to 10,000 packets, ensuring that the segments still generate the relevant alerts. Finally, we re-run Snort on these refined segments to verify that the same alerts are still produced, thus confirming the integrity of the segmentation process. To create the scenarios and questions, we generate a sample set by using two complementary approaches to address different aspects of analyst workflows: \textit{alert triaging} and \textit{deep-dive investigation}. Alert triaging evaluates the model's ability to quickly classify alerts as false positives or true positives, which is critical for prioritizing analyst workload and reducing time spent on benign activities. Deep-dive investigation assesses whether LLMs can be misled by false positive scenarios when asked to perform detailed analysis of benign artifacts, testing their resilience against confirmation bias and their ability to correctly conclude that suspicious-looking traffic is actually benign.

\noindent\emph{\underline{Alert Triaging}}: Alert triaging determines whether generated alerts represent genuine security threats or benign network activity.

\noindent\textbf{Scenario Generation}: We incorporate alert descriptions directly into scenarios while maintaining consistency with our attack dataset tone. Example: \textit{``The SOC team has received the following alert: 07/07-08:00:50.818009 [**] [122:1:1] (port\_scan) TCP portscan [**] [Priority: 3] \{TCP\} 192.168.10.3:88 - 192.168.10.5:49175. A PCAP file has been provided to investigate the alert.''}
 % Each scenario follows the format: \textit{``The SOC team has received the following alert: [alert description]. A PCAP file has been provided to investigate the alert.
    
\noindent\textbf{Question Format:} Each scenario includes one direct question: \textit{``Determine if the generated alert is a false positive or true positive.''}

\noindent\textbf{Ground Truth Labeling:} We analyze alert descriptions and corresponding attacker/victim IP addresses to establish truthfulness. True positive samples receive the label \textit{True Positive}, while false positive samples are labeled \textit{False Positive}.

\noindent\textbf{Artifact}: Corresponding segmented PCAP files related to each alert are provided to the LLM for analysis.

\noindent\emph{\underline{Deep-Dive Investigation}}: Deep-dive investigation mirrors our SIA dataset design approach, requiring comprehensive analysis of benign network artifacts.

\noindent\textbf{Scenario Generation:} To maintain consistency with our SIA dataset design approach, we transform alert descriptions into scenarios with similar tone and abstraction level. Rather than including concrete alert details (e.g. IP addresses, timestamps, port numbers), we extract key behavioral indicators and craft abstract descriptions that mirror our SIA dataset scenarios. We employ Gemini 1.5 Flash \cite{Google_AI} for initial scenario generation using few-shot learning \cite{ma2023fairness} with example scenarios from SIA dataset, the generated alert, and general instructions. Each generated scenario undergoes manual validation and adjustment to ensure alignment with our SIA dataset tone. Example: The alert \textit{``07/07-08:00:50.818009 [**] [122:1:1] (port\_scan) TCP portscan [**] [Priority: 3] \{TCP\} 192.168.10.3:88 -> 192.168.10.5:49175''} becomes: \textit{An analyst detects unusual network activity suggesting that an internal host is scanning another internal system, raising concerns of potential port scanning activity. A PCAP file, capture.pcap, has been provided to determine if this is benign network behavior or an indicator of compromise.}

\noindent\textbf{Question Format:} We design three distinct questioning approaches for deep-dive investigation, each targeting different aspects of LLM reasoning and bias detection:

\begin{itemize}[leftmargin=*, itemsep=0pt, topsep=0pt]
    \item \textbf{Assumption-Based Questions}: Inspired and aligned with blue team training platforms, these questions assume the incident's validity and seek direct investigative details. They presuppose malicious activity and request specific evidence (IPs, files, etc.). Example: \textit{What is the IP address responsible for conducting the port scan activity?}
    
    \item \textbf{Reasoning-First Questions}: Aligned with our debiasing approach taken in developing SIA dataset, these questions prompt LLMs to assess incident validity before providing details. They encourage critical analysis rather than assumption. Example: \textit{Is there any indication of port scanning activity in the network traffic? If so, what is the IP address?}
    
    \item \textbf{Validation-Only Questions}: These questions test whether LLMs are influenced by evidence-seeking prompts by focusing solely on incident truthfulness without requesting specific indicators. Example: \textit{Is there any indication of port scanning activity in the network? Answer with yes/no.}
\end{itemize}

\noindent\textbf{Ground Truth Labeling:} As for deep-dive investigation, the alerts are generated from benign samples, The ground truth for each query is set to \textit{no such entity.}

\noindent\textbf{Artifact}: Corresponding segmented PCAP files related to each alert are provided to the LLM for analysis.

% In summary, for our CIC-IDS 2017 dataset evaluation, we generated X true positive alerts and Y false positive alerts for alert triaging. For deep-dive investigation, we developed 10 scenarios based on false positive alerts, resulting in 40 investigative questions covering tasks such as victim/attacker IP identification, scan type classification, file extraction, information leakage detection, and command execution analysis.



\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Benchmark}} & \textbf{TS} & \textbf{TQ} & \textbf{Details}                                                                                             \\ \hline
Our Work                                 & 21          & 192         & \begin{tabular}[c]{@{}c@{}}21 scenarios\\ 192  questions\end{tabular} \\ \hline
PentestGPT \cite{deng2024pentestgpt}                               & 13          & 182         & \begin{tabular}[c]{@{}c@{}}13 vulnerable machines\\ 182 subtasks\end{tabular}                                \\ \hline
InterCode-CTF \cite{yang2023language}                           & 100         & 100         & 100 challenges                                                                                               \\ \hline
CyBench \cite{zhang2024cybench}                               & 40          & 40          & 100 challenges                                                                                               \\ \hline
AutoPenBench \cite{gioacchini2024autopenbench}                           & 33          & 33          & \begin{tabular}[c]{@{}c@{}}22 in-vitro or basic tasks\\ 11 real CVE based tasks\end{tabular}                 \\ \hline
\end{tabular}
}
\footnotesize{TS = Total Scenarios; TQ = Total Questions}
\caption{Comparison of different cybersecurity benchmarks}
\label{tab:dataset_scale_comparison}
\end{table}

In summary, our SIA dataset comprises 21 cyber incident scenarios with a total of 192 questions as showed in Table \ref{tab:scenario_summary}, designed to evaluate LLM capabilities across a range of security incident analysis (SIA) tasks with varying complexity. Overall, our dataset scale aligns with previous works such as \cite{deng2024pentestgpt, zhang2024cybench, gioacchini2024autopenbench, yang2023language} as showed in Table \ref{tab:dataset_scale_comparison}. The dataset is publicly available at: \url{https://github.com/llmslayer/SIA\_Dataset}.

And for exploring the LLMs capability in analysing benign artifacts, our evaluation using the CIC-IDS 2017 dataset has \textbf{X} true positive and \textbf{Y} false positive alert scenarios for alert triaging. For a deep-dive investigation, we crafted 10 scenarios, generating 39 questions focused on investigative questions such as, attacker and victim IP identification, scan classification, file extraction, leaked data information, command execution analysis.

